Structural Complexities of Matching Mechanisms

We study various novel complexity measures for two-sided matching mechanisms, applied to the two canonical strategyproof matching mechanisms, Deferred Acceptance (DA) and Top Trading Cycles (TTC). Our metrics are designed to capture the complexity of various structural (rather than computational) concerns, in particular ones of recent interest within economics. We consider a unified, flexible approach to formalizing our questions: Define a protocol or data structure performing some task, and bound the number of bits that it requires. Our main results apply this approach to four questions of general interest; for mechanisms matching applicants to institutions, our questions are: (1) How can one applicant affect the outcome matching? (2) How can one applicant affect another applicant's set of options? (3) How can the outcome matching be represented / communicated? (4) How can the outcome matching be verified? Holistically, our results show that TTC is more complex than DA, formalizing previous intuitions that DA has a simpler structure than TTC. For question (2), our result gives a new combinatorial characterization of which institutions are removed from each applicant's set of options when a new applicant is added in DA; this characterization may be of independent interest. For question (3), our result gives new tight lower bounds proving that the relationship between the matching and the priorities is more complex in TTC than in DA. We nonetheless showcase that this higher complexity of TTC is nuanced: By constructing new tight lower-bound instances and new verification protocols, we prove that DA and TTC are comparable in complexity under questions (1) and (4). This more precisely delineates the ways in which TTC is more complex than DA, and emphasizes that diverse considerations must factor into gauging the complexity of matching mechanisms.

==> omitted-proofs.tex <==



\subsection{Complexity of Verifying Counting}
\label{sec:complexity-verifying-counting}

First, we formally define the more standard notion of a verification protocol in the context of non-matching problems.

\begin{definition}
  \label{def:public-outcome-verif}
  A (public-outcome) \emph{verification protocol} of a function $f : \T_1\times\ldots\times\T_n\to A$ is defined by a set $\Certs$, a function $\mathsf{outcome}:\Certs \to A$, and a profile of functions $(\check_d)_{d \in \{1,\ldots,n\}}$, where $\check_d : \T_d \times \Certs \to \{0,1\}$ such that:
  \begin{enumerate}
    \item (Completeness) For every $t = (t_d)_{d\in\{1,\ldots,n\}} \in \T$, there exists a $C \in \Certs$ such that $f(t) = \mathsf{outcome}(C)$, and $\check_d(t_d,C)=1$ for each $d\in\{1,\ldots,n\}$.
    \item (Soundness) For every $t = (t_d)_{d\in\{1,\ldots,n\}} \in \T$ and $A \ne f(t)$, if $C \in \Certs$ is such that $A = \mathsf{outcome}(C)$ over $R$, then $\check_d(t_d,C)=0$ for at least one $d\in\{1,\ldots,n\}$.
  \end{enumerate}
      
  The \emph{cost} of a verification protocol is $\log_2|\Certs|$.
  The \emph{(public-outcome) verification complexity} of a function $f$ is the minimum of the cost of all (public-outcome) verification protocols for $f$. 
\end{definition}

\begin{definition}
  The \emph{bit-counting} function has, for some number of players $n$, input sets $\T_i = \{0,1\}$ for each $i=1,\ldots,n$, outcome set $A = \{0,1,\ldots,n\}$, and outcome function $f(b_1,\ldots,b_n) = \sum_{i=1}^n b_i$.
\end{definition}

In the proof of \autoref{thrm:verif-lb-both-mechs}, we showed than any verification protocol for $\TTC$ or for any stable matching mechanism could be used to define a (public-outcome) verification protocol for the bit-counting problem, with no increase in verification cost. We now show that the verification cost of the bit-counting problem is nearly as high as possible:

\begin{proposition}
  \label{thrm:complexity-verifying-counting}
  The verification complexity of bit-counting with $n$ players is $\Omega(n)$.
\end{proposition}
\begin{proof}
  For convenience, suppose that $n$ is a multiple of $2$.
  Let $\mathcal{F} \subseteq \{0,1\}^n$ denote the set of inputs $\vec{b} = (b_1,\ldots,b_n)$ such that $\sum_{i=1}^n b_i = \nicefrac{n}{2}$. We will show that for any verification protocol for bit-counting, we have $|\Certs| \ge |\mathcal{F}|$. 
  To prove this, suppose for contradiction that $|\Certs| < |\mathcal{F}|$. Observe that two distinct $\vec{b}, \vec{b}' \in \mathcal{F}$ must then correspond to the same certificate $C \in \Certs$. Now, let $j \in \{1,\ldots,n\}$ be any index such that ${b}_j\ne{b}'_j$, and define $\vec{b}''$ such that ${b}''_j = {b}'_j$ and ${b}''_i = {b}_i$ for each $i\ne j$. Then, we have $\check_i(b_i'', C) = 1$ for each $i \in \{1,\ldots,n\}$, since each value of $b_i''$ is equal to either $b_i$ or $b_i'$.
  But we also have that $\mathsf{outcome}(C) = \sum_{i=1}^n b_i \ne \sum_{i=1}^n b_i''$, so the verification protocol must violate soundness. This is a contradiction, showing that $|\Certs|\ge|\mathcal{F}|$.

  Thus, the verification complexity of bit-counting is at least $\log|\mathcal{F}| = \log{\binom{n}{n/2}} = \Omega(n)$.
\end{proof}


\subsection{Deterministic Blackboard Protocol for \texorpdfstring{$\TTC$}{TTC}}
\label{sec:deterministic-blackboard-ttc}



The following simple protocol mentioned in \autoref{sec:verif-complexity} may be folklore: 

\begin{theorem}
  \label{thrm:deterministic-cc-ttc}
  There is a deterministic, blackboard communication protocol for $\TTC$ (even in a model in which the priorities are not known in advance by the applicants) with communication cost $\widetilde O\bigl(|\Appls|\bigr)$.
\end{theorem}
\begin{proof}
  The protocol proceeds in steps, with one applicant or institution acting per step. First, the protocol selects an arbitrary institution $h_1$, which announces its top choice applicant $d_1$ and points to it. Then, $d_1$ announces her top institution $h_2$ and points to it. Then, $h_2$ announces and points, etc. This continues, with the protocol keeping track of some tentative chain $h_1\to d_1\to h_2\to d_2\to \cdots \to h_k \to d_k$, until some cycle is found, say $d_k \to h_j$ for some $j \in \{1,2,\ldots,k\}$. Every applicant in the cycle is permanently matched to the institution to which it points, and the applicants are removed from the market (and the capacities of these institutions are each reduced by $1$). Then, if $j > 1$, this process resumes, starting from $d_{j-1}$ pointing to her top ranked institution with remaining capacity.

  If each applicant had only pointed once during this protocol, our desired communication bound would have followed immediately. While applicants may point more than once, an applicant points a second time \emph{at most once for each cycle that is matched}. Since each cycle permanently matches at least one applicant, there are at most $|\Appls|$ matched cycles overall, and thus there are at most $O\bigl(|\Appls|\bigr)$ occurrences where an applicant is called to point, and thus the protocol uses $\widetilde O\bigl(|\Appls|\bigr)$ bits of communication overall.
\end{proof}


\subsection{Verification Protocol for \texorpdfstring{$\APDA$}{APDA} and \texorpdfstring{$\IPDA$}{IPDA}}
\label{sec:details-verifying-da}

We now prove the following result from \autoref{sec:verif-complexity}:
\restateThrmVerifComplexityDa*
The remainder of this section is dedicated to the proof.  First, note that the lower bound is given in \autoref{thrm:verif-lb-both-mechs}.

For the upper bound, it suffices to consider balanced markets with $n = |\Appls| = |\Insts|$, and prove that the verification complexity in this market is $\widetilde O(n)$. To see why, observe that the outcome of $\APDA$ (or $\IPDA$) in a many-to-one market corresponds to the outcome in the one-to-one market where every institution $h \in \Insts$ in the original market is replaced by institutions $h^1,h^2,\ldots,h^{q_h}$ (each with priority list identical to $h$'s, and where $h$ is replaced on each applicant's preference list by $h^1\succ h^2\succ\ldots\succ h^{q_h}$). Thus, a verification protocol with cost $\widetilde O\bigl(|\Appls|\bigr)$ for many-to-one markets can be defined by running a verification protocol on the corresponding one-to-one market, and for the rest of this section we focus on one-to-one markets. Thus, for the rest of this section, we assume that $n = |\Appls| = |\Insts|$.

We now define the main concept needed for our verification protocols, the ``improvement graphs.''  This definition is closely related to notions from \cite{GusfieldStableStructureAlgs89}, the standard reference work on the lattice properties of the set of stable matchings, and we will crucially use their results in our proof of correctness below.

\begin{definition}
  \label{def:improvement-graphs}
  Consider any one-to-one matching market with priorities $Q$ and preferences $P$, and consider any matching $\mu$.

  First, define a directed graph $\ImprGrI = \ImprGrI(Q,P,\mu)$. The vertices of $\ImprGrI$ are all applicants $d \in \Appls$. The edges of $\ImprGrI$ are all those pairs $(d, d')$ such that there exists $h\in\Insts$ such that $h\ne\emptyset$ is the highest institution on $d$'s preference list such that $d \succ_h \mu(h)$, and moreover $\mu(h) = d'$. For such a $d, d', h$, we denote this edge by $d \xrightarrow{h} d'$.
   

  
  Second, define a directed graph $\ImprGrA = \ImprGrA(Q,P,\mu)$ with precisely the same definition as $\ImprGrI$, except interchanging the roles of applicants and institutions. 
\end{definition}

Observe that the vertices of each of $\ImprGrI$ and $\ImprGrA$ have out-degree at most $1$, and thus these graphs take only $\widetilde O(n)$ bits to describe.

Our key lemma will show next that a matching equals $\IPDA$ if and only if $\ImprGrI$ is acyclic.
To begin to gain intuition for this, observe that if $\mu$ is stable and $d \xrightarrow{h} d'$ is an edge in $\ImprGrI$, then $h$ must be below $\mu(d)$ on $d$'s preference list.
Informally, the lemma will follow because edges in $\ImprGrI$ represent possible ways matches could be exchanged that make the matching better for the applicants and worse for the institutions, and cycles in $\ImprGrI$ characterize such changes to the matching that could be accomplished without violating stability. 
\begin{lemma}
  \label{thrm:improvement-graphs-show-opt}
  Fix any set of preferences $P$ and priorities $Q$. For any matching $\mu$, we have $\mu = \IPDA_Q(P)$ if and only if both $\mu$ is stable with respect to $P$ and $Q$ and the graph $\ImprGrI(Q,P,\mu)$ is acyclic.
  Dually, $\mu = \APDA_Q(P)$ if and only if both $\mu$ is stable and $\ImprGrA(Q,P,\mu)$ is acyclic.
\end{lemma}
\begin{proof}
  We prove the first result, namely, that $\IPDA$ is characterized by $\ImprGrI$. The proof relies heavily on results from \cite[Section 2.5.1]{GusfieldStableStructureAlgs89}. % ; for completeness and clarity, we provide the full details relying only on lattice properties of the set of stable matchings.
  First, observe that in the language of \cite{GusfieldStableStructureAlgs89}, the edges $d\xrightarrow{h} d'$ of $\ImprGrI$ are exactly those $d,h,d'$ such that $h = s_\mu(d)$ and $d' = \mathit{next}_{\mu}(d)$.%
  \footnote{%
    \label{footnote:GI-outdegree-error}%
    We remark that \cite[Section 2.5.1, Page 87]{GusfieldStableStructureAlgs89} mentions the following: ``Note that $s_\mu(d)$ might not exist. For example, if $\mu$ is the [institution]-optimal [stable] matching, then $s_\mu(d)$ does not exist for any [applicant] $d$.'' The second sentence of this quote would seem to eliminate the need for our verification protocol to communicate any graph whatsoever, since if $\mu = \IPDA$, then this graph should be empty. However, the claim made in passing in that second sentence is false. For example, if 
    $h_1 : d_1\succ d_2$, 
    $h_2 : d_2\succ d_1$, 
    $h_a : d_1\succ d_2 \succ d_3$, and
    $d_1 : h_2 \succ h_a \succ h_1$,
    $d_2 : h_1 \succ h_a \succ h_2$,
    $d_3 : h_a$,
    then $\mu = \IPDA = \{ (d_1,h_2), (d_2,h_1), (d_3,h_a) \}$, and $s_\mu(d_1) = s_\mu(d_2) = h_a \ne \emptyset$. (Note that $s_\mu(d_3) = \emptyset$, and thus our graph $\ImprGrI$ has edges $d_1 \to d_3 \leftarrow d_2$, and is indeed acyclic.)
  }
  
  First, we show that if $\mu$ is stable and $\ImprGrI$ has a cycle, then $\mu \ne \IPDA = \IPDA_Q(P)$. Suppose $d_1 \xrightarrow{h_1} d_2 \xrightarrow{h_2} d_3 \xrightarrow{h_3} \ldots  \xrightarrow{h_{k-1}} d_k \xrightarrow{h_k} d_1$ is some cycle in $\ImprGrA$. Then, according to the definitions given in \cite[Page 88]{GusfieldStableStructureAlgs89}, we have that $\rho = [ (d_1,h_{k}), (d_2,h_1), \ldots, (d_k, h_{k-1}) ]$ is a rotation exposed in $\mu$. Define a matching $\mu'$ such that $\mu'(d_i) = h_{i}$ for each $i=1,\ldots,k$ (with indices mod $k$), and $\mu'(d) = \mu(d)$ for all $d$ not contained in the above cycle (in the language of \cite{GusfieldStableStructureAlgs89}, we have $\mu' = \mu / \rho$, the elimination of rotation $\rho$ from $\mu$). \cite[Lemma 2.5.2]{GusfieldStableStructureAlgs89} shows that $\mu' \ne \mu$ is also stable, and is preferred by all institutions to $\mu$. Thus, by the fact that $\IPDA$ is the institution-optimal stable outcome, we have $\mu \ne \IPDA$.
  

  Second, we show that if $\mu$ is stable and $\mu \ne \IPDA_Q(P)$, then $\ImprGrI$ must have a cycle. By \cite[Lemma 2.5.3]{GusfieldStableStructureAlgs89}, there is some rotation $\rho = [ (d_1,h_{k}), (d_2,h_1), \ldots, (d_k, h_{k-1}) ]$ that is exposed in $\mu$. By the definition of $\ImprGrI$ and the definition of a rotation from \cite{GusfieldStableStructureAlgs89}, this rotation corresponds to a cycle $d_1 \xrightarrow{h_1} d_2 \xrightarrow{h_2} d_3 \xrightarrow{h_3} \ldots  \xrightarrow{h_{k-1}} d_k \xrightarrow{h_k} d_1$ in $\ImprGrI$.%
  \footnote{
    In fact, our $\ImprGrI$ is defined in a way very close to the graph $H(\mu)$ which \cite{GusfieldStableStructureAlgs89} consider in the proof of their Lemma 2.5.3; our graph $\ImprGrI$ simply considers the entire set of applicants, instead of just those who have a different partner in $\mu$ and $\IPDA \ne \mu$, and our graph generalizes theirs to arbitrary matchings $\mu$, possibly including $\IPDA$ (which fixes the minor error mentioned in \autoref{footnote:GI-outdegree-error}).
    }
  So $\ImprGrI$ is cyclic.

  Since $\ImprGrA$ is defined precisely by interchanging the roles of applicants and institutions, we have that $\ImprGrA$ characterizes $\APDA$ in the same way.
\end{proof}

Now, we can define a verification protocol $V^\IPDA$ (resp.\ $V^\APDA$) for $\IPDA$ (resp.\ $\APDA$). 
When priorities are $Q$ (recall that the priorities $Q$ are known to each applicant before the mechanism begins\footnote{
  Several steps of this protocol (both checking stability and checking the correctness of the graph $\ImprGrI$ or $\ImprGrA$) would require $\Omega(n^2)$ bits if priorities are not known to the applicants, cf.\ \cite{GonczarowskiNOR19}.
}) and preferences are $P$, the certificate $C$ records the matching $\mu = \IPDA_Q(P)$ (resp.\ $= \APDA_Q(P)$) and graph $G = \ImprGrI$ (resp.\ $= \ImprGrA$). By \autoref{thrm:improvement-graphs-show-opt}, it suffices for the applicants to collectively verify that the matching $\mu$ is stable, and that the graph $G$ is correctly constructed.
As already noted in \autoref{sec:verif-complexity},
it is not hard to verify that $\mu$ is stable once $\mu$ is known: each applicant $d$ can identify using $\mu$ and $Q$ which institutions $h$ are such that $d \succ_h \mu(h)$ according to $Q$, and each applicant can simply check that there are no such $h$ where $h \succ_d \mu(d)$. Thus, to complete the proof, it suffices to show the following lemma:

\begin{lemma}
  \label{lem:exist-predicates-checking-graph}
  If priorities $Q$ are fixed ahead of time, there exists a predicate $\check_d(P_d,\mu,G) \in \{0,1\}$ for each $d\in\Appls$, such that for all preferences $P$, matchings $\mu$, and graphs $G$, we have:
  \[ \bigwedge_{d \in \Appls} \check_d(P_d,\mu,G) = 1
  \quad \iff \quad
  G = \ImprGrI(Q,P,\mu).\]
  Moreover, the same claim holds (with a different predicate $\check_d(\cdot)$) replacing $\ImprGrI$ with $\ImprGrA$.
\end{lemma}
\begin{proof}
  We first prove the claim for $\ImprGrI$. This case is not too hard to see: each $d$ just needs to verify that the edge outgoing from her node in $G$ exactly corresponds to $d\xrightarrow{h} d'$, where $d'=\mu(h)$ and $h$ is $d$'s highest-ranked institution such that $d \succ_h \mu(h)$ (if it exists). Since $d$ knows the priorities, $d$ also knows the set of all $h$ such that $d \succ_h \mu(h)$, and can thus perform this verification. % since the priorities of each $h$ are common knowledge

  We now prove the claim for $\ImprGrA$, which requires a somewhat more delicate predicate $\check_d(\mu,G)$. For clarity, note that the full definition of $\ImprGrA$ is as follows:
  There is a vertex for each $h \in \Insts$, and an edge $h \xrightarrow{d} h'$ whenever $h,h',d$ are such that both $\mu(d)=h'$ and $d \ne \emptyset$ is the highest-ranked applicant on $h$'s preference list such that $h \succ_d \mu(d)$. We claim that it suffices for each applicant $d$'s predicate $\check_d(\mu,G)$ to verify all of the following:
  \begin{itemize}
    \itemsep0em
    \item For each edge $h_x \xrightarrow{d} h_y$, we have $h_x \succ_d h_y = \mu(d)$.
    \item For each edge $h_x \xrightarrow{d_y} h_y$ with $d_y \ne d$: if we let $d_x = \mu(h_x)$, then whenever $d_x \succ_{h_x} d \succ_{h_x} d_y$ according to the priorities $Q$, we have $\mu(d) \succ_d h_x$.
    \item For each $h$ with out-degree zero in $G$, we have $\mu(d)\succ_d h$.
  \end{itemize}
  The first condition is necessary for each $d$ by the definition of $\ImprGrA$. 
  If the first and second condition are both true for every $d\in\Appls$, then every edge in $G$ is correctly constructed according to $\ImprGrA$, because if these conditions hold then each $d_y$ in some edge $h_x\xrightarrow{d_y} h_y$ is the highest-ranked applicant below $d_x=\mu(h_x)$ such that $h_x \succ_{d_y} \mu(d_y)$. Finally, the third condition for every $d \in \Appls$ guarantees that an institution has out-degree zero in $G$ if and only if it has out-degree zero according to $\ImprGrA$.
  This shows that $G = \ImprGrA$ if and only if each of the above three predicates is true for each $d \in \Appls$, as desired. Since the above conditions can be verified for each $d$ using only knowledge of the priorities, $\mu$, $G$, and $d$'s own preferences, this proves the lemma.
\end{proof}

This finishes the proof of \autoref{thrm:verif-complexity-da}: the verification protocols $V^\IPDA$ and $V^\APDA$ communicate a certificate containing the matching $\mu$ and corresponding graph $G$ that requires only $\widetilde O(n) = \widetilde O\bigl(|\Appls|\bigr)$ bits, and applicants check that $\mu$ is stable and that the graph is correctly constructed as above.

\begin{remark}
  \label{remark:score-based-model}
  While our model (and our lower bounds) assume that the entire priority lists of each institution are known to all applicants, all of the protocols we mention or construct \autoref{sec:protocol-complexity} can actually be implemented with a more mild assumption on the knowledge of the priorities. 
  Assume that there are scores $e_h^d \in [0,1]$  for each $d\in\Appls$ and $h\in\Insts$, and let $d \succ_h d'$ if and only if $e_h^d > e_h^{d'}$.
  Assume that each applicant $d$ starts off knowing $\bigl\{ e_h^d \bigr\}_{h \in \Insts}$, but any other information must be communicated through the certificate $C$.
  First, observe that the protocols adapted from \cite{AzevedoL16} and \cite{LeshnoL21} in \autoref{sec:compression-complexity} work exactly as written.
  
  Now, consider the verification protocol for $\TTC$ from \autoref{thrm:verif-complexity-ttc}. This verification protocol can still post a transcript of the deterministic protocol for $\TTC$ from \autoref{thrm:deterministic-cc-ttc}, since that deterministic protocol works even when the priorities must be communicated. However, note that the institutions are not agents participating in the protocol, so the institutions cannot themselves take part in the verification of the transcript of the protocol. Thus, every time that an institution $h$ points to an applicant $d$ during the transcript, the protocol should also announce the priority score of applicant $d$ at institution $h$; and each applicant who is not yet matched in the transcript should check that they do not have higher priority at $h$. This suffices to verify the transcript of the deterministic protocol.

  For $\DA$, an analogous trick works. When the protocol to verify $\IPDA$ posts certificate $\mu, \ImprGrI$, it should also post the priority scores of $\mu(h)$ at $h$ for each $h \in \Insts$, and applicants will still be able to verify each edge $d \xrightarrow{h} d'$ in $\ImprGrI$, as in \autoref{lem:exist-predicates-checking-graph}.
  When the protocol to verify $\APDA$ posts certificate $\mu, \ImprGrA$, it should also post, for every edge $h\xrightarrow{d}h'$, the priority scores of $d$ at both $h$ and $h'$. Then, again each applicant knows what she needs in order to perform the verification as in \autoref{lem:exist-predicates-checking-graph}.
\end{remark}

\begin{remark}
  While \autoref{thrm:verif-complexity-da} holds for both $\APDA$ and $\IPDA$, it cannot be extended to any matching mechanism. To see why, consider a market with applicants $d^0_1,\ldots,d^0_n, d_1^1,\ldots,d_n^1$ and institutions $h_1^0,\ldots,h_n^0, h_1^1,\ldots,h_n^1$, where each applicant and institution has a full-length preference list. Suppose each institution $h_i^j$ for $i\in\{1,\ldots,n\}$ and $j \in \{0,1\}$ ranks $d_i^j$ first and ranks $d_i^{1-j}$ last, 
  with any fixed order between them. Now consider the set of preferences where each applicant $d_i^j$ for $i\in\{1,\ldots,n\}$ and $j \in \{0,1\}$ ranks $h_i^{1-j}$ first and ranks $d_i^{j}$ last, where any possible ordering over the other institutions appears between first and last. Observe that, for any profile of preferences in this class, the matchings $\mu_0 = \bigl\{ (d_i^j, h_i^j) \bigr\}_{i \in \{1,\ldots,n\}, j \in \{0,1\}}$ and $\mu_1 = \bigl\{ (d_i^j, h_i^{1-j}) \bigr\}_{i \in \{1,\ldots,n\}, j \in \{0,1\}}$ are both stable. Thus, consider a stable matching mechanism $f$ that (on inputs in this class) outputs either $\mu_0$ or $\mu_1$, depending on some arbitrary function $g : \T \to \{0,1\}$ of the preference lists of the $2n$ applicants, and suppose that the function $g$ has verification complexity $\Omega(n^2)$ (such a function can be constructed by standard techniques using a counting argument). Then, the verification complexity of $f$ will be at least the verification complexity of $g$, i.e., $\Omega(n^2)$.
\end{remark}


